A Fast Parameterized Algorithm for Co-Path Set

The k-CO-PATH SET problem asks, given a graph G and a positive integer k, whether one can delete k edges from G so that the remainder is a collection of disjoint paths. We give a linear-time fpt algorithm with complexity O^*(1.588^k) for deciding k-CO-PATH SET, significantly improving the previously best known O^*(2.17^k) of Feng, Zhou, and Wang (2015). Our main tool is a new O^*(4^{tw(G)}) algorithm for CO-PATH SET using the Cut&Count framework, where tw(G) denotes treewidth. In general graphs, we combine this with a branching algorithm which refines a 6k-kernel into reduced instances, which we prove have bounded treewidth.

==> analysis.tex <==




%There are two stages of our algorithm where we are selecting edges to be in $F$. First we randomly remove edges which are incident to vertices with degree greater than or equal to six, resulting in a graph $G'$ with maximum degree at most five. We denote $F$ upon completion of the this random removal step as $F_1$ and we let $k_1 = k' - |F_1|$. Thus the size of our five-capping-edge sets are $k_1$. We restrict all of these edge sets to be of the same size for one run in \textsc{C\&C:Co-Path}.By Lemma \ref{lem31}, the \textsc{Parameterized Co-Path Set} problem is equivalent on $K$ and $G'$ with probability $(2/3)^{k_1}$. 

%We will refer to this entire process as the \textit{kernelization} step. Note that we iterate over all possible $k + 1$ values of $k_1$, each value corresponds to one run in \textsc{C\&C:Co-Path}. This guarantees that we find a co-path set of size $k$ if one exists. As our graph is assumed to be simple there are at most $n^2$ edges in the graph. Thus we can write the $k$ coefficient which arises in to the abbreviated polynomial $n$ term, and our computation complexity is solely dependent on the running time of one run of \textsc{C\&C:Co-Path}. 

%Next we run the Cut\&Count algorithm on $G'$. We are able to remove $k' - k_1$ edges from $G'$, thus we will look for a solution which has $|E(G')| - k' + k_1$ edges. We say there are $k_2$ edges added to $F$ during Cut\&Count. Note that $k' = k_1 + k_2$. 


%HERE

%Analysis of kernelization

%Each kernelization takes $O(k_1)$ time.    As we use randomization in finding $G'$, we must calculate the probability of making the correct selections in this step. By Theorem \ref{thm:constantprob}, after $c * 1.5^{k_1}$ total operations over all kernelizations, the probability that no $F_1$ has led to a solution is constant. Thus with high probability we will have found a $F_1$ that leads to a solution, if one exists. 
    
   
   %If we do not have an $F_1$ that leads to a solution, we can conclude that our initial assumption is false and no solution exists. Note that the number of times we run the kernelization step is $(c_1 * 1.838^{k_1})$.
%Given an instance of $G'$, by Theorems \ref{our_tw} and \ref{cutcount} Cut\&Count determines whether a solution exists in time $O^*(1.588^{k_2})$. As Cut\&Count is deterministic, it runs once for each kernelizing run. We say \textsc{RCC} is a run consisting of one kernelizing run followed by one run of Cut\&Count. Thus, one run of \textsc{RCC} takes time $O^*(k_1 + 1.588^{k_2})$. 

%One run of \textsc{C$\&$C: Co-Path} consists of all $c_1 * 1.5^{k_1}$ runs of \textsc{RCC}. Thus \textsc{C$\&$C: Co-Path} operates in $O^*(1.588^k)$, as $k_1 + k_2 = k$, and have shown Theorem \ref{main} to be true. 













\iffalse
For all connected components which are cycles we remove one edge and add it to $F$. Then we contract all thin paths in $G'$, yielding $G''$. Lastly we contract all edges linking a degree 1 vertex with a degree 2 vertex, resulting in $G'''$. 


By Lemma \ref{lem31}, the \textsc{Parameterized Co-Path Set} problem is equivalent on $K$ and $G'$ with probability $(2/3)^{k_1}$.  Next we run the Cut\&Count alogrithm on the graph $G'$ which is yielded by the kernelization step. We are able to remove $k - k_1$ edges from $G'''$, thus we will look for a solution which has $|E(G''')| - k + k_1$ edges .  We say there are $k_2$ edges added to $F$ during Cut\&Count. Note that as we know the size of $F$ is $k$, and there are $k_1$ edges added to $F$ during kernelization and $k_2$ edges added to $F$ during Cut\&Count, $k = k_1 + k_2$. 

Each kernelization takes $O(k_1)$ time. As we use randomization in finding $G'$, we must calculate the probability of making the correct selections in this step. After $c * 1.5^{k_1}$ total operations over all kernelizations, the probability that no $F_1$ has led to a solution is less than or equal to $(1/e)^c$. Thus with high probability we will have found a $F_1$ that leads to a solution, if one exists. If we have not an $F_1$ that leads to a solution, we can conclude with high probability that our initial assumption is false and no solution exists. Note that the number of times we run the kernelization step is $(c_1 * 1.5^{k_1}) / (c_2 * k_1)$.

Given an instance of $G'''$, by Theorems 4.1 and 5.2 Cut\&Count determines whether a solution exists in time $O^*(1.588^{k_2})$. As Cut\&Count is deterministic, it runs once for each kernelizing run. We say \textsc{RCC} is a run consisting of one kernelizing run followed by one run of Cut\&Count. Thus, one run of \textsc{RCC} takes time $O^*(k_1 + 1.588^{k_2})$. 

The algorithm \textsc{C$\&$C: Co-Path} consists of all $(c_1 * 1.5^{k_1})$ runs of \textsc{RCC}. \textsc{C$\&$C: Co-Path} operates in $O^*(1.588^k)$, as $k_1 + k_2 = k$. Thus we have shown Theorem 1.1 to be true. 


\fi
